Oracle-Efficient Differentially Private Learning with Public Data

Due to statistical lower bounds on the learnability of many function classes under privacy constraints, there has been recent interest in leveraging public data to improve the performance of private learning algorithms. In this model, algorithms must always guarantee differential privacy with respect to the private samples while also ensuring learning guarantees when the private data distribution is sufficiently close to that of the public data. Previous work has demonstrated that when sufficient public, unlabelled data is available, private learning can be made statistically tractable, but the resulting algorithms have all been computationally inefficient. In this work, we present the first computationally efficient, algorithms to provably leverage public data to learn privately whenever a function class is learnable non-privately, where our notion of computational efficiency is with respect to the number of calls to an optimization oracle for the function class. In addition to this general result, we provide specialized algorithms with improved sample complexities in the special cases when the function class is convex or when the task is binary classification.

==> body/regression.tex <==
\section{Follow The Regularized Leader}


\begin{algorithm}
    \begin{algorithmic}[1]
    \State \textbf{Input } ERM oracle $\erm$, perturbation parameter $\eta > 0$, integer $m$, data set $\cD = \left\{ (X_i, Y_i) | 1 \leq i \leq n \right\}$, function class $\cF$, loss function $\ell$, noise level $\gamma > 0$, hallucinating distribution $\mu$. \\
    \hrulefill
    \State \textbf{Generate } $\cDtil = \left\{ Z_1, \dots, Z_m \right\}$  such that $Z_i \sim \mu$.
    \State \textbf{Define } $\Omega: \cF \to \rr$ such that
    \begin{equation}\label{eq:Omega}
        \Omega(f) = \sum_{(X_i, Y_i) \in \cD } \ell(f(X_i), Y_i) + \eta \cdot \norm{f(Z)}_{m}^2.
    \end{equation}
    \State \textbf{Set } $\fbar = \erm(\Omega, \cF)$
    \State \textbf{Sample} $\xi_1, \dots, \xi_m \sim \cN(0, 1)$.
    \State \textbf{Define } $R: \cF \to \rr$ such that
    \begin{equation}
        R(f) = \norm{f - \fbar - \gamma \cdot \xi}_{m}^2.
    \end{equation}
    \State \textbf{Output } $\fhat = \erm(R, \cF)$.
    \end{algorithmic}
    \caption{Oracle Efficient Private Learner}
    \label{alg:dp_alg}
 \end{algorithm}
The following is our main result:
\begin{theorem}
    Let $\fhat$ be defined as in \Cref{alg:dp_alg} with $\cD$ sampled independently from some distribution $\nu$ and suppose that $\norm{\frac{d \nu_x}{d \mu}}_{\infty} \leq \frac 1\sigma$.  Suppose the loss function $\ell$ is convex, $\lambda$-Lipschitz, and bounded uniformly by $1$ in the first argument, the function class $\cF$ is convex, and $L(f) = \ee_{(X, Y) \sim \nu}\left[ \ell(f(X), Y) \right]$.  If $\log \cN(\cF, \epsilon) \leq d \log\left( \frac 1\epsilon \right)$, then setting
    \begin{align}
        \gamma = \frac{\alpha \sigma}{\sqrt{\log\left( \frac 1\beta \right)}}, && m = \frac{d \log\left( \frac 1\beta \right)}{\sigma^2 \alpha^2}, && \eta = \frac{d \log^{2}\left( \frac 1\beta \right)}{\alpha^3 \sigma^3 \epsilon} \vee \frac{d \log^{3/2}\left( \frac 1\beta \right) \cdot \log^{1/2}\left( \frac 1\delta \right)}{\alpha^2 \sigma^2 \epsilon}
    \end{align}
    yields an $(\epsilon, \delta)$-differentially private $(\alpha, \beta)$-learner as long as
    \begin{align}
        n \geq \Omega\left( \frac{d \log^{2}\left( \frac 1\beta \right)}{\alpha^4 \sigma^3 \epsilon} \vee \frac{d \log^{3/2}\left( \frac 1\beta \right) \cdot \log^{1/2}\left( \frac 1\delta \right)}{\alpha^3 \sigma^2 \epsilon} \vee \frac{\lambda^2 d}{\alpha^2} \vee \frac{\log\left( \frac 1\beta \right)}{\alpha^2}\right).
    \end{align}
\end{theorem}
\abcomment{Also observe that we can replace uniform bound on Radon-Nikodym derivative by membership in $f$-divergence ball by my results with Yury.}  \abcomment{Also observe that at the cost of adding polynomial factors in $\alpha$, we can move to pure differential privacy by replacing Gaussian noise with exponential noise.} \abcomment{also observe that result holds for nonparametric $\cF$ with different rates.}
The theorem follows from the following two propositions:
\begin{proposition}\label{prop:privacy}
    \abcomment{add in linear dependence in $\lambda$ and propagate through to final result}
    If $\cA$ is \Cref{alg:dp_alg}, $\cF$ is convex, and
    \begin{align}
        \frac{m}{\gamma^2 \eta} + \frac{m}{\gamma \eta} \cdot \sqrt{\log\left( \frac 1 \delta \right)} \leq \epsilon,
    \end{align}
    then $\cA$ is $(\epsilon, \delta)$-differentially private.
\end{proposition}
\begin{proof}
    To ease notation, fix $\cD, \cD'$ adjacent data sets and let $\fbar, \fbar'$ denote the minimizers of $\Omega, \Omega'$ respectively, where $\Omega$ is as in \eqref{eq:Omega} and $\Omega'$ is defined similarly, but replacing $\cD$ by $\cD'$.  Similarly, let $\fhat, \fhat'$ be the result of applying $\cA$ to $\cD, \cD'$.  By \Cref{lem:l2_stability}, it holds that $\norm{\fbar - \fbar'}_m \leq \frac{4 \lambda}{\eta}$.  Let $\cB_\delta$ denote the event that $\norm{\xi}_m \leq \gamma \cdot \sqrt{\log\left( \frac 1\delta \right)}$ and note that $\pp(\cB_\delta) \geq 1 - \delta$.  To proceed, denote by $\pp_u$ the distribution of $\cA(\cD)$ conditioned on $\fbar + \xi = u$ and denote $\pp_u'$ similarly.  Furthermore, let
    \begin{align}
        p_{\cD}(u) = (2 \pi \sigma^2)^{- \frac m2} \exp\left( - \frac{m \norm{u - \fbar}_m^2}{2 \gamma^2 } \right) 
    \end{align}
    be the distribution of $u$ given $\fbar$ and define $p_{\cD'}(u)$ similarly.  Then we may compute:
    \begin{align}
        \pp\left( \cA(\cD) \in \cG \right) &= \int_{u \in \rr^m} \pp_u\left( \cA(\cD) \in \cG \right) p_{\cD}(u) d u \\
        &= \int_{u} \bbI[\cB_\delta ] \pp_u\left( \cA(\cD) \in \cG \right) p_{\cD}(u) d u \\
        &\quad + \int_u \bbI[\cB_\delta^c ] \pp_u\left( \cA(\cD) \in \cG \right)  p_{\cD}(u) d u \\
        &\leq \delta + \int_{u} \bbI[\cB_\delta ] \pp_u\left( \cA(\cD) \in \cG \right) p_{\cD}(u) d u. \\
        &= \delta + \int_{u} \bbI[\cB_\delta ] \pp_u'\left( \cA(\cD') \in \cG \right) p_{\cD}(u) d u,
    \end{align}
    where the last equality follows from the fact that $\cA(\cD')$ is conditionally independent of $\cD'$ given $\fbar'$.  Now, for the second term, we observe that
    \begin{align}
        \int_{u} \bbI[\cB_\delta ] \pp_u'\left( \cA(\cD') \in \cG \right) p_{\cD}(u) d u &= \int_{u} \bbI[\cB_\delta ] \pp_u'\left( \cA(\cD') \in \cG \right) p_{\cD'}(u) \exp\left( \frac{m}{2 \gamma^2}\left( \norm{u - \fbar'}_m^2 - \norm{u - \fbar}_m^2 \right) \right) d u \\
        &\leq \int_{u} \bbI[\cB_\delta ] \pp_u'\left( \cA(\cD') \in \cG \right) p_{\cD'}(u) \exp\left( \frac{m}{\gamma^2}\left(1 + \norm{u}_m \right) \cdot \norm{\fbar - \fbar'}_m \right) d u \\
        &\leq \int_{u} \bbI[\cB_\delta ] \pp_u'\left( \cA(\cD') \in \cG \right) p_{\cD'}(u) \exp\left( \frac{m}{\gamma^2}\left(1 + \gamma \cdot \sqrt{\log\left( \frac 1\delta \right)} \right) \cdot \norm{\fbar - \fbar'}_m \right) d u \\
        &\leq e^\epsilon \cdot \int_{u} \bbI[\cB_\delta ] \pp_u'\left( \cA(\cD') \in \cG \right) p_{\cD'}(u) d u \\
        &\leq e^\epsilon \cdot \pp\left( \cA(\cD') \in \cG\right),
    \end{align}
    where the first inequality follows from the local Lipschitzness of the squared norm, the second inequality follows from the construction of $\cB_\delta$, the third inequality follows from the assumption on the paramters, and the final inequality follows from the fact that probabilities are nonnegative.  Combining these displays proves the proposition.
\end{proof}
We now control the excess risk of the algorithm:
\begin{proposition}\label{prop:excess_risk}
    Let $\cA$ be as in \Cref{alg:dp_alg} and suppose that $\norm{\frac{d \nu_x}{d \mu}}_{\infty} \leq \frac 1\sigma$.  Suppose the loss function $\ell$ is $\lambda$-Lipschitz and bounded uniformly by $1$ in the first argument, and $L(f) = \ee_{(X, Y) \sim \nu}\left[ \ell(f(X), Y) \right]$.  Letting $\ftil$ denote the ERM, it holds that
    \begin{align}
        L(\fhat) \leq L(\ftil) + \lambda \cdot \rad_n(\cF) + \frac \eta n + \sqrt{\frac{2\log\left( \frac 1 \beta \right)}{n}} + \frac C\sigma \cdot \left( \gamma  + r_m \right) \cdot \sqrt{\log\left( \frac 1\beta \right)}
    \end{align}
    with probability at least $1 - \beta$.
\end{proposition}
\begin{proof}
    Define
    \begin{align}
        \Lnhat(f) = \frac 1n \cdot \sum_{(X_i, Y_i) \in \cD} \ell(f(X_i), Y_i),
    \end{align}
    and let $\ftil \in \argmin_{f \in \cF} \Lnhat(f)$ be the ERM.  Observe that
    \begin{align}
        \Lnhat(\fbar) + \frac \eta n \cdot \norm{\fbar}_m^2 \leq \Lnhat(\ftil) + \frac \eta n \cdot \norm{\ftil}_m^2.
    \end{align}
    Because $\norm{\ftil}_m^2 \leq 1$, this implies that
    \begin{align}\label{eq:fbar_erm_bound}
        \Lnhat(\fbar) \leq \Lnhat(\ftil) + \frac \eta n.
    \end{align}
    On the other hand, \abcomment{cite}, with probability at least $1 - \beta$, it holds that for all $f \in \cF$,
    \begin{align}
        \abs{\Lnhat(f) - L(f)} \leq \lambda \cdot \rad_n(\cF) + \sqrt{\frac{2\log\left( \frac 1 \beta \right)}{n}},
    \end{align}
    where $\rad_n(\cF)$ is the Rademacher complexity \abcomment{define somewhere}.  Thus,
    \begin{align}
        L(\fbar) \leq L(\ftil) + \lambda \cdot \rad_n(\cF) + \frac{\eta}{n} + \sqrt{\frac{2\log\left( \frac 1 \beta \right)}{n}}.
    \end{align}
    To conclude, we observe that
    \begin{align}
        L(\fhat) &\leq L(\fbar) + L(\fhat) - L(\fbar) \\
        &\leq L(\fbar) + \lambda \cdot \norm{\fhat - \fbar}_{L^2(\nu)} \\
        &\leq L(\fbar) + \frac{\lambda}{\sigma} \cdot \norm{\fhat - \fbar}_{\mu}.
    \end{align}
    Now, with probability at least $1 - \beta$, it holds that for all $f, f' \in \cF$,
    \begin{align}
        \norm{f - f'}_{\mu} \leq C \cdot \norm{f - f'}_m  + r_m \cdot \sqrt{\log\left( \frac 1 \beta \right)},
    \end{align}
    where $r_m$ is the critical radius \abcomment{cite and explain how this scales like $\sqrt{d/m}$ for what we care about.}.  Finally, observe that
    \begin{align}
        \norm{\fhat - \fbar}_m \leq 2 \cdot \norm{\xi}_m \leq 2 \gamma \cdot \sqrt{\log\left( \frac 1 \beta \right)},
    \end{align}
    with probability at least $1 - \beta$.  The result follows.
    
    The result follows.
\end{proof}




\subsection{Auxiliary Lemma}

\begin{lemma}\label{lem:l2_stability}
    Suppose that $\ell$ is convex and $\lambda$-Lipschitz in its first argument.  Let $\cD, \cD'$ denote data sets differing in a single entry and let $\fbar, \fbar'$ dentoe the minimizers of $\Omega, \Omega'$ from \eqref{eq:Omega}.  If $\cF$ is convex, then,
    \begin{align}
        \norm{\fbar - \fbar'}_{m} \leq \frac{4\lambda}{\eta}.
    \end{align}
\end{lemma}
\begin{proof}
    To see this, note that by strong convexity of the squared norm and convexity of $\cF$, it holds that
    \begin{align}
        \Omega'(\fbar') \geq \Omega(\fbar) + \frac{\eta}{2} \norm{\fbar - \fbar'}_m^2.
    \end{align}
    On the other hand,
    \begin{align}
        \Omega(\fbar') &= \Omega'(\fbar') + \Omega(\fbar') - \Omega'(\fbar') \\
        &\leq \Omega'(\fbar) + \Omega(\fbar') - \Omega'(\fbar') \\
        &= \Omega(\fbar) + \Omega(\fbar') - \Omega'(\fbar') + \Omega'(\fbar) - \Omega(\fbar) \\
        &\leq \Omega(\fbar) + 2 \lambda \cdot \norm{\fbar-  \fbar'}_m.
    \end{align}
    Combining this with the previous display and rearranging yields:
    \begin{align}
        \eta \cdot \norm{\fbar - \fbar'}_m^2 \leq 4 \lambda \cdot \norm{\fbar - \fbar'}_m.
    \end{align}
    Rearranging again proves \eqref{eq:l2_stability}.
\end{proof}


\section{Follow the Perturbed Leader}

In this section we present a different algorithm that allows for weaker conditions on the loss function and $\cF$, but requires a stronger oracle.  In particular, given function class $\cF$, function $f_0 \in \cF$, distance $d$ and radius $\alpha$, we let
\begin{align}
    \erm\left( L, \cF, f_0, \alpha \right) \in \argmin_{\substack{f \in \cF \\ d(f, f_0) > \alpha}} L(f).
\end{align}
\begin{algorithm}
    \begin{algorithmic}[1]
    \State \textbf{Input } ERM oracle $\erm$, perturbation parameter $\eta > 0$, integer $m$, data set $\cD = \left\{ (X_i, Y_i) | 1 \leq i \leq n \right\}$, function class $\cF$, loss function $\ell$, noise level $\gamma > 0$, radius $\rho > 0$, hallucinating distribution $\mu$. \\
    \hrulefill
    \State \textbf{Generate } $\cDtil = \left\{ Z_1, \dots, Z_m \right\}$  such that $Z_i \sim \mu$.
    \For{$j = 1, 2, \dots$}
        \State \textbf{Sample} $\xi_1, \dots, \xi_m \sim \cN(0, 1)$.
        \State \textbf{Define } $\omega_m: \cF \to \rr$ such that
        \begin{equation}
            \omega_m(f) = \frac 1{\sqrt m} \cdot \sum_{i = 1}^m \xi_i \cdot f(Z_i).
        \end{equation}
        \State \textbf{Define } $\Omega: \cF \to \rr$ such that
        \begin{equation}
            \Omega(f) = \sum_{(X_i, Y_i) \in \cD } \ell(f(X_i), Y_i) + \eta \cdot \omega_m(f).
        \end{equation}
        \State \textbf{Set } $\fbar = \erm(\Omega, \cF)$ and $\ftil = \erm(\Omega, \cF, \fbar, \rho)$.
        \If{$\Omega(\ftil) > \Omega(\fbar) + 1$}
            \State \textbf{Break}
        \EndIf
    \EndFor
    \State \textbf{Sample} $\xi_1, \dots, \xi_m \sim \cN(0, 1)$.
    \State \textbf{Define } $R: \cF \to \rr$ such that
    \begin{equation}
        R(f) = \norm{f - \fbar - \gamma \cdot \xi}_{m}^2.
    \end{equation}
    \State \textbf{Output } $\fhat = \erm(R, \cF)$.
    \end{algorithmic}
    \caption{Oracle Efficient Private Learner (Gaussian Perturbation)}
    \label{alg:dp_alg_ftpl}
 \end{algorithm}
\begin{theorem}\label{thm:ftpl}
    Suppose that $\cF: \cX \to [-1,1]$ is a function class \abcomment{all measurability assumptions satisfied} and suppose that $\log \cN(\cF, \epsilon) \leq d \log\left( \frac 1\epsilon \right)$ \abcomment{observe that result holds for nonparametric function classes too but different bounds}.  Suppose that $\ell: [-1,1]^{\times 2} \to [0,1]$ is a loss function continuous in the first argument.  Let $\mu \in \Delta(\cX)$ denote a measure such that $\inf_{f \in \cF} \norm{f}_{\mu} \geq \frac 12$ and suppose that $\norm{\frac{d \nu_x}{\mu}}_\infty \leq \frac 1\sigma$.  If we set
    \begin{align}
        \gamma = \frac{\alpha \sigma}{\sqrt{\log\left( \frac 1\beta \right)}}, && m = \frac{d \log\left( \frac 1\beta \right)}{\sigma^2 \alpha^2},  && \rho = \frac{\epsilon \alpha^4 \sigma^4}{d \log^2\left( \frac 1\beta \right)} \wedge \frac{\epsilon \alpha^3 \sigma^3}{d \log\left( \frac 1\beta \right) \sqrt{\log\left( \frac 1\delta \right)}} \\
    \end{align}
    and
    \begin{align}
        \eta = C \left(\frac{2 d^{5/2} \log^4\left( \frac 1\beta \right)}{\epsilon^2 \alpha^8 \sigma^8} \vee \frac{2 d^{5/2} \log^2\left( \frac 1\beta \right) \log\left( \frac 1\delta \right)}{\epsilon^2 \alpha^6 \sigma^6}\right),
    \end{align}
    then \Cref{alg:dp_alg_ftpl} is an $(\epsilon, \delta)$-differentially private $(\alpha, \beta)$-learner as long as
    \begin{align}
        n \geq \Omega\left( \frac{\lambda^2 d}{\alpha^2} \vee \frac{d \log\left( \frac 1\beta \right)}{\alpha^2} \vee \frac{d^3 \log^4\left( \frac 1\beta \right) \log\log\left( \frac 1\beta \right)}{\epsilon^2 \alpha^9 \sigma^8} \vee \frac{d^3 \log^2\left( \frac 1\beta \right) \log\left( \frac 1\delta \right) \log\log\left( \frac 1\beta \right)}{\epsilon^2 \alpha^7 \sigma^6} \right)
    \end{align}
    Furthermore, with probability at least $1 - \beta$, \Cref{alg:dp_alg_ftpl} requires $O\left( \log\left( \frac 1\beta \right) \right)$ calls to the ERM oracle.
\end{theorem}
We first observe that the requirement that $\inf_{f \in \cF} \norm{f}_{\mu}$ is easy to satisfy.  Indeed, we may introduce an auxiliary point $Z^\star$ such that $f(Z^\star) = 1$ for all $f \in \cF$ and let $\mutil = \frac 12 \cdot \mu + \frac 12 \delta_{Z^\star}$.  Then we see that $\norm{\frac{d \nu_x}{d \mutil}}_\infty \leq 2 \cdot \norm{\frac{d \nu_x}{d \mu}}_\infty$ and $\inf_{f \in \cF} \norm{f}_{L^2(\mutil)} \geq \frac 12$.  In fact, because the contribution of these points to $\Omega$ is independent of $f$, we may assume this purely in the analysis.
\begin{proof}
    We first bound the number of iterations of the loop in \Cref{alg:dp_alg_ftpl}.  Indeed, by boundedness \Cref{prop:gaussiananticoncentration}, it holds that for each iteration of the loop for any $\rho, \tau > 0$,
    \begin{align}
        \pp\left( \inf_{\norm{f - \fbar}_m > \rho} \Omega(f) < \Omega(\fbar) + \tau \right) \leq \frac{8}{\rho^2 \kappa^2 \eta} \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right] \leq C \frac{\sqrt{d}}{\rho^2 \eta}.
    \end{align}
    Let $\cA_J$ denote the event that the loop runs for at least $J$ iterations.  Then, by independence, it holds that
    \begin{align}
        \pp\left( \cA_J \right) = \left( C \frac{\sqrt{d}}{\rho^2 \eta} \right)^J
    \end{align}
    and thus with probability at least $1 - \beta$, the loop runs for at most
    \begin{align}
        J = C \cdot \frac{\log\left( \frac 1\beta \right)}{\log\left( \frac{ \sqrt {d}}{\rho\eta} \right)}
    \end{align}
    iterations, as long as $C \frac{\sqrt{d}}{\rho^2 \eta} < 1$.

    As in the proof of \Cref{prop:privacy} \abcomment{convert sensitivity bound to privacy bound in lemma and then refer to this in both places}, we have that if
    \begin{align}
        \frac{m\rho}{\gamma^2} + \frac{m\rho}{\gamma} \cdot \sqrt{\log\left( \frac 1 \delta \right)} \leq \epsilon,        
    \end{align}
    then \Cref{alg:dp_alg_ftpl} is $(\epsilon, \delta)$-differentially private by applying \Cref{prop:gaussiananticoncentration}.  Thus, setting


    As in the proof of \Cref{prop:excess_risk} and with the same notation from that section \abcomment{at some point just make a single lemma for the perturbation and use it in both places}, we have that
    \begin{align}
        L(\fhat) \leq L(\ftil) + \lambda \cdot \rad_n(\cF) + \sqrt{\frac{2 \log\left( \frac 1\beta \right)}{n}} + \frac{C}{\sigma}\left( \gamma + r_m \right) \cdot \sqrt{\log\left( \frac 1\beta \right)} +  \frac \eta n \cdot \max_{1 \leq j \leq J} \sup_{f \in \cF} \omega_m^{(j)}(f),
    \end{align}
    where the only difference is that we have replaced the perturbation term.  We now observe that with probability at least $1 - \beta$, it holds that
    \begin{align}
        \sup_{f \in \cF} \omega_m(f) \leq C \left( \sqrt{d + \frac{\log\left(\frac 1 \beta \right)}{m}} \right)
    \end{align}
    and thus with probability at least $1 - \beta$,
    \begin{align}
        \max_{1 \leq j \leq J} \sup_{f \in \cF} \omega_m^{(j)}(f) \leq C \left( \sqrt{d + \log\left( \frac J \beta \right)} \right).
    \end{align}
    The result follows by plugging in the parameters in the statement of the theorem.
\end{proof}









\begin{proposition}\label{prop:gaussiananticoncentration}
    Let $\cF: \cX \to [-1,1]$ be a function class and let $\ell: [-1,1] \times [-1,1] \to [0,1]$ be a (measurable) loss function.  Let $\mu \in \Delta(\cX)$ denote a measure such that $\inf_{f \in \cF} \norm{f}_{\mu} \geq \kappa$.  Let $\cD, \cD'$ denote data sets differing in a single entry, let
    \begin{align}
        \omega_m(f) = \frac 1{\sqrt m} \cdot \sum_{i = 1}^m \xi_i \cdot f(Z_i)
    \end{align}
    for $Z_i \sim \mu$ and $\xi_i \sim \cN(0, 1)$ independent.  Let
    \begin{align}
        \Omega(f) = L_{\cD}(f) + \eta \cdot \omega_m(f)
    \end{align}
    and $\Omega'$ defined similarly and further denote by $\fbar, \fbar'$ the minimizers of $\Omega, \Omega'$.  Then,
    \begin{align}
        \pp\left( \inf_{\norm{f - \fbar}_m > \rho} \Omega(f) < \Omega(\fbar) + 1 \right) \leq \frac{8}{\rho^2 \kappa^2 \eta} \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right].
    \end{align}
    In particular,
    \begin{align}
        \pp\left( \norm{\fbar - \fbar'}_{m} > \rho \right) \leq \frac{8}{\rho^2 \kappa^2 \eta} \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right]
    \end{align}
    and
    \begin{align}
        \ee\left[ \norm{\fbar - \fbar'}_m \right] \leq \frac{2 \sqrt{2 \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right]}}{\kappa \sqrt{\eta}}.
    \end{align}
\end{proposition}
\begin{proof}
    Note that by boundedness of $\ell$, it holds that
    \begin{align}
        \sup_{f \in \cF} \abs{L_{\cD}(f) - L_{\cD'}(f)} \leq 1.
    \end{align}
    The first claim is \Cref{lem:gaussiananticoncentration2} and the second claim follows immediately after observing that
    \begin{align}
        \ee\left[ \sup_{f \in \cF} \Omega(f) - \ee\left[ \Omega(f) \right] \right] = \eta \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right].
    \end{align}
    For the third claim, note that for any $\zeta > 0$, it holds that
    \begin{align}
        \ee\left[ \norm{\fbar - \fbar'}_m \right] &\leq \zeta + \int_\zeta^1 \pp\left( \norm{\fbar - \fbar'}_m > \rho \right) d \rho \\
        &\leq \zeta + \int_\zeta^1 \frac{8}{\rho^2 \kappa^2 \eta} \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right] d \rho \\
        &\leq \zeta + \frac{8}{\kappa^2 \eta \zeta} \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right].
    \end{align}
    Minimizing over $\zeta$ proves the claim.
\end{proof}


\subsection{Algorithm with Standard ERM Oracle}

Here we return to the standard ERM oracle where for $L: \cF \to \rr$ we let $\erm(L, \cF) = \fstar$ denote a minimizer of $L$ over $\cF$.  We now present a variant of \Cref{alg:dp_alg_ftpl} that succeeds even with this oracle.
\begin{algorithm}
    \begin{algorithmic}[1]
    \State \textbf{Input } ERM oracle $\erm$, perturbation parameter $\eta > 0$, integer $m$, data set $\cD = \left\{ (X_i, Y_i) | 1 \leq i \leq n \right\}$, function class $\cF$, loss function $\ell$, noise level $\gamma > 0$, number of iterations $J > 0$, hallucinating distribution $\mu$. \\
    \hrulefill
    \State \textbf{Generate } $\cDtil = \left\{ Z_1, \dots, Z_m \right\}$  such that $Z_i \sim \mu$.
    \For{$j = 1, 2, \dots, J$}
        \State \textbf{Sample} $\xi_1^{(j)}, \dots, \xi_m^{(j)} \sim \cN(0, 1)$.
        \State \textbf{Define } $\omega_m: \cF \to \rr$ such that
        \begin{equation}
            \omega_m^{(j)}(f) = \frac 1{\sqrt m} \cdot \sum_{i = 1}^m \xi_i \cdot f(Z_i).
        \end{equation}
        \State \textbf{Define } $\Omega: \cF \to \rr$ such that
        \begin{equation}
            \Omega^{(j)}(f) = \sum_{(X_i, Y_i) \in \cD } \ell(f(X_i), Y_i) + \eta \cdot \omega_m^{(j)}(f).
        \end{equation}
        \State \textbf{Set } $\fbar_j = \erm(\Omega^{(j)}, \cF)$
    \EndFor
    \State \textbf{Define} $\fbar = \frac 1J \cdot \sum_{j = 1}^J \fbar_j$. 
    \State \textbf{Sample} $\xi_1, \dots, \xi_m \sim \cN(0, 1)$.
    \State \textbf{Define } $R: \cF \to \rr$ such that
    \begin{equation}
        R(f) = \norm{f - \fbar - \gamma \cdot \xi}_{m}^2.
    \end{equation}
    \State \textbf{Output } $\fhat = \erm(R, \cF)$.
    \end{algorithmic}
    \caption{Oracle Efficient Private Learner (Gaussian Perturbation)}
    \label{alg:dp_alg_ftpl2}
 \end{algorithm}
\begin{theorem}
    Suppose that $\cF: \cX \to [-1,1]$ is a function class \abcomment{all measurability assumptions satisfied} and suppose that $\log \cN(\cF, \epsilon) \leq d \log\left( \frac 1\epsilon \right)$ \abcomment{observe that result holds for nonparametric function classes too but different bounds}.  Suppose that $\ell: [-1,1]^{\times 2} \to [0,1]$ is a loss function continuous in the first argument.  Let $\mu \in \Delta(\cX)$ denote a measure such that $\inf_{f \in \cF} \norm{f}_{\mu} \geq \frac 12$ and suppose that $\norm{\frac{d \nu_x}{\mu}}_\infty \leq \frac 1\sigma$.  If we set
    \begin{align}
        \gamma = \frac{\alpha \sigma}{\sqrt{\log\left( \frac 1\beta \right)}}, && m = \frac{d \log\left( \frac 1\beta \right)}{\sigma^2 \alpha^2},  && J = 
    \end{align}
    \abcomment{change parameters}
    and
    \begin{align}
        \eta = C \left(\frac{2 d^{5/2} \log^4\left( \frac 1\beta \right)}{\epsilon^2 \alpha^8 \sigma^8} \vee \frac{2 d^{5/2} \log^2\left( \frac 1\beta \right) \log\left( \frac 1\delta \right)}{\epsilon^2 \alpha^6 \sigma^6}\right),
    \end{align}
    \abcomment{change parameters}
    then \Cref{alg:dp_alg_ftpl2} is an $(\epsilon, \delta)$-differentially private $(\alpha, \beta)$-learner as long as
    \begin{align}
        n \geq \Omega\left( \frac{\lambda^2 d}{\alpha^2} \vee \frac{d \log\left( \frac 1\beta \right)}{\alpha^2} \vee \frac{d^3 \log^4\left( \frac 1\beta \right) \log\log\left( \frac 1\beta \right)}{\epsilon^2 \alpha^9 \sigma^8} \vee \frac{d^3 \log^2\left( \frac 1\beta \right) \log\left( \frac 1\delta \right) \log\log\left( \frac 1\beta \right)}{\epsilon^2 \alpha^7 \sigma^6} \right)
    \end{align}
    \abcomment{change parameter} that requires only \abcomment{include J +1 scaling} calles to the ERM oracle.
\end{theorem}
\begin{proof}
    The proof is almost identical to that of \Cref{thm:ftpl} with the exception that we now need to bound $\rho$ in terms of $J$ with high probability.  To do this, we begin by applying Jensen's and noting that for any $\rho > 0$,
    \begin{align}
        \pp\left( \norm{\fbar - \fbar'}_m > \rho \right) &= \pp\left( \norm{\frac 1J \sum_{j = 1}^J \fbar_j - \fbar_j'}_m > \rho \right) \\
        &= \pp\left( \norm{\frac 1J \sum_{j = 1}^J \fbar_j - \fbar_j'}_m^2 > \rho^2 \right) \\
        &\leq \pp\left( \frac 1J \sum_{j = 1}^J  \norm{\fbar_j - \fbar_j'}_m^2 > \rho^2 \right).
    \end{align}
    Now, we observe that because $\norm{\fbar_j - \fbar_j'}_m \leq 2$ for all $j$, it holds by a Hoeffding's inequality that
    \begin{align}
        \pp\left( \frac 1J \sum_{j = 1}^J  \norm{\fbar_j - \fbar_j'}_m^2 >  \ee\left[ \norm{\fbar_1 - \fbar_1'}_m \right] + \sqrt{\frac{\log\left( \frac 1\delta \right)}{J}} \right) \leq \delta.
    \end{align}
    By \Cref{lem:gaussiananticoncentration3}, we have that
    \begin{align}
        \ee\left[ \norm{\fbar_1 - \fbar_1'}_m \right] \leq \frac{32}{\kappa^2 \eta} \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right] \cdot \log\left( \eta \kappa^2 \ee\left[ \sup_{f \in \cF} \omega_m(f) \right]\right).
    \end{align}
    Thus, if 
    \begin{align}
        J \geq \left(\frac{32}{\kappa^2 \eta} \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right] \cdot \log\left( \eta \kappa^2 \ee\left[ \sup_{f \in \cF} \omega_m(f) \right]\right)\right)^2 \log\left( \frac 1\delta \right),
    \end{align}
    then with probability at least $1 - \delta$, it holds that
    \begin{align}
        \norm{\fbar - \fbar'}_m \leq \sqrt{\frac{C}{\kappa^2 \eta} \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right] \cdot \log\left( \eta \kappa^2 \ee\left[ \sup_{f \in \cF} \omega_m(f) \right]\right)\log\left( \frac 1\delta \right)}.
    \end{align}
    \abcomment{finish plugging in parameters to get final bound.}
\end{proof}
\begin{lemma}\label{lem:gaussiananticoncentration3}
    Suppose we are in the situation of \Cref{prop:gaussiananticoncentration}.  Then,
    \begin{align}
        \ee\left[ \norm{\fbar - \fbar'}_m^2 \right] \leq \frac{32}{\kappa^2 \eta} \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right] \cdot \log\left( \eta \kappa^2 \ee\left[ \sup_{f \in \cF} \omega_m(f) \right]\right).
    \end{align}
\end{lemma}
\begin{proof}
    We compute for any $\zeta > 0$, using \Cref{prop:gaussiananticoncentration},
    \begin{align}
        \ee\left[ \norm{\fbar - \fbar'}_m^2 \right] &\leq \zeta + \int_\zeta^1 2 \rho \pp\left( \norm{\fbar - \fbar'}_m > \rho \right) d \rho \\
        &\leq \zeta + 2 \cdot \int_\zeta^1 \rho \cdot \frac{8}{\rho^2 \kappa^2 \eta} \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right] d \rho \\
        &\leq \zeta + \frac{16}{\kappa^2 \eta} \cdot \ee\left[ \sup_{f \in \cF} \omega_m(f) \right] \cdot \log\left( \frac 1\zeta \right).
    \end{align}
    Minimizing over $\zeta$ proves the claim.
\end{proof}
















\subsection{Gaussian Anti-Concentration}


\abcomment{Include discussion on why minimizer is almost surely unique.}
% \begin{lemma}\label{lem:gaussiananticoncentration}
%     Let $T$ be a set, $m: T \to \rr$ be a mean function and $K: T \times T \to \rr$ be a covariance kernel (in the sense of being positive definite).  Let $d$ denote the metric induced by $K$ and suppose that $m$ is continuous  with respect to $d$, and the metric space $(T, d)$ is separable and compact.  Let $\omega$ denote a Gaussian process on $T$ with covariance $K$ and for $\eta > 0$, let
%     \begin{align}
%         \Omega(t) = m(t) + \eta \cdot \omega(t)
%     \end{align}
%     be an offset Gaussian process.  We further suppose that $\omega$ is taken to be a version with almost surely continuous paths $t \mapsto \omega(t)$ and that $0 < \kappa \leq K(t,t) \leq 1$ for all $t \in T$.  Let
%     \begin{equation}
%         \tstar = \argmin_{t \in T} \Omega(t),
%     \end{equation}
%     and,
%     \begin{equation}
%         \cE(\rho, \tau) = \left\{\text{there exists } s \in T \text{ such that } \frac{K(s,t)}{K(t,t)} \leq 1 - \rho^2 \text{ and } \Omega(s) \leq \Omega(\tstar) + \tau \right\},
%     \end{equation}
%     for $\rho, \tau > 0$.  The following holds:
%     \begin{align}
%         \pp\left(\cE(\rho, \tau)\right) \leq  \frac{\tau}{\rho^2 \eta^2 \kappa^2} \cdot \ee\left[\sup_{t \in T} \Omega(t) - m(t)\right].
%     \end{align}
% \end{lemma}
% \begin{proof}
%     Note that by compactness of $T$ and almost sure continuity of $\Omega$, $\tstar$ exists almost surely.  As $T$ is separable and $\Omega$ has almost surely continuous sample paths, it suffices to replace $T$ with a countable dense subset.  We will hereafter suppose without loss of generality that $T$ is countable.  For each $t \in T$, define the set
%     \begin{align}
%         A(t) = \left\{s \in T \bigg| \frac{K(s, t)}{K(t,t)} \leq 1 - \rho^2 \text{ and } \Omega(s) \leq \Omega(t) + \tau  \right\}.
%     \end{align}
%     It then suffices to lower bound the probability that $A(\tstar) = \emptyset$.  We compute
%     \begin{align}
%         \pp\left(\abs{A(\tstar)} = 0 \right) &= \sum_{t \in T} \pp\left(\tstar = t \text{ and } \abs{A(t)} = 0\right) \\
%         &= \sum_{t \in T} \ee_y\left[\pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq (1 - \rho^2)K(t,t)} \Omega(s) \geq y + \tau| \Omega(t) = y\right) \right],
%     \end{align}
%     where the expectation is taken over the distribution of $\Omega(t)$.  Now, fix $t$ and let $\Omega_{t,y}$ denote the Gaussian process $\Omega$ conditioned on the event that $\Omega(t) = y$.  Let $m_{t,y}$ and  $\eta^2 \cdot K_t$ denote the mean and covariance processes of $\Omega_{t,y}$.  Critically, note that $K_t$ is independent of $y$ and for all $s \neq t$, we have
%     \begin{align}
%         m_{t,y}(s) = m(s) + \frac{K(s, t)}{K(t,t)}\left(y - m(t)\right).
%     \end{align}
%     Define the functions
%     \begin{align}
%         a(s) = \frac \tau{\rho^2} \cdot \frac{K(s, t) }{ K(t,t)}  \qquad \text{ and } \qquad b(s) = \frac{\tau}{\rho^2}  - a(s).
%     \end{align}
%     Now, note that if $K(s, t) \leq (1 - \rho^2)\cdot K(t,t)$, then
%     \begin{align}\label{eq:conditionalineq1}
%         b(s)  = \frac{\tau}{\rho^2}\left(1 - \frac{K(s, t)}{ K(t,t)}\right)  \geq \frac{\tau}{\rho^2 } \cdot \rho^2 = \tau.
%     \end{align}
%     We also have that $b(s) \geq 0$ for all $s$ by the fact that $K(s,t) \leq \sqrt{K(s,s) \cdot K(t,t)}$ and $K(s,s) \vee K(t,t) \leq 1$.  Furthermore, for all $s$, it holds that
%     \begin{equation}\label{eq:conditionalineq2}
%         m_{t, y + \frac{\tau}{\rho^2}}(s) = m_{t,y}(s) + a(s).
%     \end{equation}
%     Thus, for fixed $t \in T$ and $y \in \rr$, we have
%     \begin{align}
%         \pp&\left(\tstar = t \text{ and } \inf_{K(s, t) \leq (1 - \rho^2)K(t,t)} \Omega(s) \geq y + \tau| \Omega(t) = y\right) \\
%         &\geq \pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq (1 - \rho^2)K(t,t)} \Omega(s) - b(s) \geq y| \Omega(t) = y\right) \\
%         &= \pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq (1 - \rho^2)K(t,t)} \Omega(s) - b(s) - a(s) + a(s) \geq y| \Omega(t) = y\right) \\
%         &= \pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq (1 - \rho^2)K(t,t)} \Omega(s) + a(s) \geq y + \frac{\tau}{\rho^2}| \Omega(t) = y\right) \\
%         &= \pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq (1 - \rho^2)K(t,t)} \Omega(s) \geq y + \frac{\tau}{\rho^2}| \Omega(t) = y + \frac{\tau}{\rho^2}\right) \\
%         &\geq \pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq (1 - \rho^2)K(t,t)} \Omega(s) \geq y + \frac{\tau}{\rho^2}| \Omega(t) = y + \frac{\tau}{\rho^2}\right),
%     \end{align}
%     where the first inequality follows from \eqref{eq:conditionalineq1}, the second equality follows from the construction, and the last equality follows from \eqref{eq:conditionalineq2} and the fact that $K_t$ is independent of $y$.  Now, denote
%     \begin{equation}
%         q_t(y) = (2 \pi K(t,t) )^{- \frac 12} \exp\left(- \frac{(y - m(t))^2}{2 \eta^2 K(t,t)}\right),
%     \end{equation}
%     the density of $\Omega(t)$ and note that we have
%     \begin{align}
%         \pp\left(\abs{A(\tstar)} = 0\right)&= \sum_{t \in T} \int_{-\infty}^\infty q_t(y) \pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq 1 - \rho^2} \Omega(s) \geq y + \tau| \Omega(t) = y\right) d y \\
%         &\geq \sum_{t \in T} \int_{\infty}^\infty q_t(y)\pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq 1 - \rho^2} \Omega(s) \geq y + \frac{\tau}{\rho^2}| \Omega(t) = y + \frac{\tau}{\rho^2}\right) d y. \label{eq:gaussianmanipulation1}
%     \end{align}
%     We then compute
%     \begin{align}
%         \int_{-\infty}^\infty q_t(y)&\pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq 1 - \rho^2} \Omega(s) \geq y + \frac{\tau}{\rho^2}| \Omega(t) = y + \frac{\tau}{\rho^2 }\right) dy \label{eq:gaussianaddsubtract}\\
%         &= \int_{- \infty}^\infty q_t(y)\pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq 1 - \rho^2} \Omega(s) \geq y | \Omega(t) = y \right)dy  \\
%         &+ \int_{-\infty}^\infty \left(q_t(y) - q_t\left(y - \frac{\tau}{\rho^2 }\right)\right) \cdot \pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq 1 - \rho^2} \Omega(s) \geq y | \Omega(t) = y \right) dy,
%     \end{align}
%     where we added and subtracted the first term and then made the variable substitution $y + \frac{\tau}{\rho^2} \mapsto y$ for the latter integral.  Note that
%     \begin{align}
%         \pp\left(\tstar = t \text{ and } \inf_{K(s, t) \leq 1 - \rho^2} \Omega(s) \geq y | \Omega(t) = y \right) = \pp\left(\tstar = t | \Omega(t) = y\right)
%     \end{align}
%     as $\Omega(s) \geq \Omega(\tstar)$ for all $s \in T$ by definition.  Combining this observation with \eqref{eq:gaussianmanipulation1} and \eqref{eq:gaussianaddsubtract} yields
%     \begin{align}
%         \pp\left(\abs{A(\tstar)} = 0\right) &\geq \sum_{t \in T} \int_{-\infty}^\infty q_t(y) \pp\left(\tstar = t | \Omega(t) = y\right) dy \\
%         &- \sum_{t \in T} \int_{-\infty}^\infty \left(q_t(y) - q_t\left(y - \frac{\tau}{\rho^2}\right)\right) \cdot \pp\left(\tstar = t | \Omega(t) = y\right) dy .
%     \end{align}
%     For the first term, we have
%     \begin{align}
%         \sum_{t \in T} \int_{-\infty}^\infty q_t(y) \pp\left(\tstar = t | \Omega(t) = y\right) d y &= \sum_{t \in T} \pp\left(\tstar = t\right) = 1.
%     \end{align}
%     For the second term, using the fact that $1 - e^x \leq x$ for all $x$, we have
%     \begin{align}
%         q_t(y) - q_t\left(y - \frac{\tau}{\rho^2}\right) &= q_t(y) \left(1 - \exp \left( \frac{(y - m(t))^2}{2\eta^2 K(t,t)} - \frac{\left(y - m(t) - \frac{\tau}{\rho^2}\right)^2}{2 \eta^2 K(t,t)}\right) \right) \\
%         &\leq q_t(y) \left(\frac{(y - m(t))^2}{2\eta^2 K(t,t)} - \frac{\left(y - m(t) - \frac{\tau}{\rho^2}\right)^2}{2 \eta^2 K(t,t)}  \right) \\
%         &\leq \frac{q_t(y)}{2 \eta^2 \kappa^2} \cdot \left( \frac{2 \tau}{\rho^2} (y - m(t)) \right).
%     \end{align}
%     Thus we have
%     \begin{align}
%         \pp\left(\abs{A(\tstar)} > 0\right) &= 1 - \pp\left(\abs{A(\tstar)} = 0\right) \\
%         &\leq \sum_{t \in T} \int_{-\infty}^\infty \frac{q_t(y)}{2 \eta^2\kappa^2} \cdot \left( \frac{2 \tau}{\rho^2} (y - m(t))\right) \cdot \pp\left( \tstar = t | \Omega(t) = y \right) d y \\
%         % &\leq \frac{\tau^2}{2 \eta^2\kappa^2\rho^4} + \sum_{t \in T} \int_{-\infty}^\infty \frac{q_t(y)}{2 \eta^2} \cdot \frac{2 \tau}{\rho^2} \cdot (y - m(t))\cdot \pp\left( \tstar = t | \Omega(t) = y \right) d y \\
%         &= \frac{\tau}{\rho^2 \eta^2 \kappa^2} \sum_{t \in T} \int_{-\infty}^\infty (y - m(t)) q_t(y) \pp\left( \tstar = t | \Omega(t) = y \right) d y \\
%         &= \frac{\tau}{\rho^2 \eta^2 \kappa^2} \cdot \ee\left[ \Omega(\tstar) - m(\tstar)\right] \\
%         &\leq  \frac{\tau}{\rho^2 \eta^2 \kappa^2} \cdot \ee\left[\sup_{t \in T} \Omega(t) - m(t)\right].
%     \end{align} 
%     The result follows.
% \end{proof}
As a corollary, we have the following:
% \begin{lemma}\label{lem:gaussiananticoncentration2}
%     Suppose that we are in the situation of \Cref{lem:gaussiananticoncentration} and that $T$ has an additive structure such that $d(s,t) = \sqrt{K(s-t,s-t)}$.  Let $m': T \to \rr$ denote a mean function such that $\sup_{t \in T} \abs{m(t) - m''(t)} \leq \tau$ and let $\Omega'$ denote the corresponding shifted Gaussian process.  If $t^{\star '} = \argmin_{t \in T} \Omega'(t)$, then
%     \begin{align}
%         \pp\left( d(\tstar, t^{\star'}) > \rho \right) \leq \frac{8 \tau}{\rho^2 \eta^2 \kappa^2} \cdot \ee\left[\sup_{t \in T} \Omega(t) - m(t)\right].
%     \end{align}
% \end{lemma}
% \begin{proof}
%     Note that
%     \begin{align}
%         d(s, t)^2 = K(s - t, s - t) = K(s,s) + K(t,t) - 2 K(s,t).
%     \end{align}
%     Let $M = \max(K(\tstar, \tstar), K(t^{\star '},t{\star '})) \leq 1$ and note that the above implies:
%     \begin{align}
%         d(\tstar,t^{\star '})^2 \leq 2 M \left(1 - \frac{K(t^{\star '}, t^{\star})}{M}\right).
%     \end{align}
%     Thus,
%     \begin{align}
%         \pp\left( d(\tstar, t^{\star '}) > \rho  \right) &\leq \pp\left( 2 M \left( 1 - \frac{K(\tstar, t^{\star '})}{M} \right) > \rho \right) \\
%         &\leq \pp\left( 1 - \frac{K(\tstar, t^{\star '})}{M}  > \frac \rho2 \right) \\
%         &\leq 2 \left(  \frac{\tau}{\left( \frac \rho 2 \right)^2 \eta^2 \kappa^2} \cdot \ee\left[\sup_{t \in T} \Omega(t) - m(t)\right]. \right) \\
%         &= \frac{8 \tau}{\rho^2 \eta^2 \kappa^2} \cdot \ee\left[\sup_{t \in T} \Omega(t) - m(t)\right],
%     \end{align}
%     where the last inequality follows by applying a union bound and \Cref{lem:gaussiananticoncentration} to the Gaussian processes $\Omega$ and $\Omega'$.
% \end{proof}






